SimSD: Simple Speculative Decoding in Diffusion Language Models

Diffusion large language models (dLLMs) have recently emerged as a promising alternative to autoregressive (AR) LLMs, offering faster inference through parallel or blockwise decoding. However, their masked language modeling formulation remains incompatible with standard token-level speculative decoding, one of the most effective acceleration techniques for AR models. In AR decoding, the causal mask preserves temporally valid token-level contexts, enabling a target model to verify multiple drafted tokens in a single forward pass. In contrast, dLLMs rely on mask tokens and bidirectional attention, causing the effective context to change across denoising steps and preventing direct token-level speculative verification. To bridge this gap, we propose a simple but effective speculative decoding algorithm for diffusion language models, named SimSD, which mainly adopts a plug-and-play masking strategy that equips dLLMs with temporally valid token-level contexts for speculative decoding. Our method explicitly introduces reference tokens from draft-model predictions and designs an attention mask that regulates their interaction with current-step tokens, allowing dLLMs to compute valid logits for drafted tokens in a single forward pass. This restores the key verification ability provided by causal masking in AR models while preserving the parallel decoding advantages of dLLMs. The proposed method is training-free and can be flexibly integrated with other acceleration techniques such as KV cache and blockwise decoding. Experiments on SDAR-family dLLMs across four benchmarks show that our method achieves up to 7.46x higher decoding throughput while maintaining and even improving average generation quality.

==> neurips26_dllm_causal_mask/src/figure/cross_model_figure.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/cross_model.png}
  \caption{Token-level temporal causal attention. (a) A step map assigns each token a temporal decoding order. (b) The input is arranged as prompt, data, and mask tokens, with shared temporal labels and aligned positional encoding. (c) The attention mask enforces token-level temporal causality.}
  \label{fig:cross_model}
\end{figure}

==> neurips26_dllm_causal_mask/src/figure/figure1.tex <==
\begin{figure}[t]
    \centering
    \resizebox{1.0\linewidth}{!}{
        \includegraphics{figures/figure1_main.png}
    }
    \caption{SimSD restores token-level speculative decoding for diffusion language models.
Vanilla dLLMs cannot directly support speculative decoding because bidirectional attention breaks temporal token-level contexts. SimSD adopts a temporal causal mask for supporting standard speculative verification in a single forward pass, leading to faster decoding without hurting performance.
}
    \label{fig:example}
\end{figure}

==> neurips26_dllm_causal_mask/src/figure/figure2.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/causal_mask-v8.pdf}
  \caption{Token-level temporal causal attention. (a) A step map assigns each token a temporal decoding order. (b) The input is arranged as prompt, data, and mask tokens, with shared temporal labels and aligned positional encoding. (c) The attention mask enforces token-level temporal causality.}
  \label{fig:standard-vs-causal}
\end{figure}

==> neurips26_dllm_causal_mask/src/figure/figure3_4.tex <==
\begin{figure}[h]
\centering

\begin{minipage}{0.48\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/self_draft.png}
  \caption{Self draft distribution analysis.
  We use SDAR-8B-Chat as both draft and target with $B=4$ and temperature $0$.}
  \label{fig:self_draft}
\end{minipage}
\hfill
\begin{minipage}{0.48\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/cross_model.png}
  \caption{Cross model distribution analysis.
  We use SDAR-1.7B-Chat as draft and SDAR-8B-Chat as target with $B=4$ and temperature $0$.}
  \label{fig:cross_model}
\end{minipage}

\end{figure}

==> neurips26_dllm_causal_mask/src/figure/self_draft_figure.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/self_draft.png}
  \caption{Self draft Distribution Analysis}
  \label{fig:self_draft}
\end{figure}

==> neurips26_dllm_causal_mask/src/section/1_introduction.tex <==
\section{Introduction}
Large language models (LLMs)~\citep{chowdhery2022palmscalinglanguagemodeling, hurst2024gpt, comanici2025gemini} have achieved remarkable success across a wide range of natural language processing tasks~\citep{zhao2023survey, minaee2024large}. These advances are largely driven by autoregressive (AR) Transformer architectures~\citep{vaswani2017attention}. Despite the performance, AR decoding is inherently sequential, which requires strictly performing token-by-token generation~\citep{fu2024lookahead_decoding, xia-etal-2024-unlocking}.
As an alternative, diffusion large language models (dLLMs)~\citep{NEURIPS2021_958c5305, Diffusion-LM} generate text by iteratively denoising an incomplete sentence with bidirectional attention. With a properly designed denoising schedule, dLLMs enable predicting multiple tokens at one decoding step, leading to promising parallelism and lower inference latency.

Recent commercial dLLMs~\citep{labs2025mercuryultrafastlanguagemodels,gemini_diffusion,bie2025llada2} have substantially narrowed the performance gap with state-of-the-art AR models, while demonstrating much faster inference speed with parallel or blockwise decoding~\citep{christopher2025specdiff, cheng2025sdar, pan2025blockspec, chen2026dflash}. However, further improving dLLM inference speed remains challenging because its masked language modeling design~\citep{devlin2019bert,nie2025llada} is not naturally compatible with many acceleration techniques developed for AR models, especially for the widely-used speculative decoding method~\citep{xia-etal-2024-unlocking,leviathan2023fast,chen2023speculative_sampling}. 
In AR models, the token-level causal mask ensures that every generated token remains in the context for subsequent positions. Thus, for speculative decoding in AR models, all the drafted tokens from a smaller model only require a single forward pass over their concatenated sequence to produce valid logits for all drafted tokens under their correct prefixes. This property is central to speculative decoding, where multiple possible tokens can be verified in parallel. By contrast, dLLMs rely on mask tokens to indicate unresolved positions and use bidirectional attention to condition on the visible context. Consequently, the effective input context changes across denoising or generation steps, and dLLMs cannot maintain temporally valid token-level contexts. Therefore, standard token-level speculative verification cannot be applied directly to dLLMs.

To address this limitation, we propose a simple but effective method namely \textbf{SimSD} that adopts a plug-and-play masking strategy that equips dLLMs with temporally valid token-level contexts for speculative decoding. The key idea is to construct a token-level causal structure in which each token can directly attend to other information from the additional reference context, \ie inference results from a smaller model, analogous to how AR models read in-context tokens through the causal mask. 
To this end, we explicitly add several tokens as the reference context and design an attention mask that regulates interactions between these reference context and the tokens predicted at the current step. In this way, the visible context is no longer determined only by the current masked input, but built to include both current-step tokens and reference context. This restored temporal context allows a dLLM to compute logits for drafted tokens and thereby supports standard speculative verification in a single forward pass. It matches the verification mechanism used in AR speculative decoding, and gives dLLMs the key ability while retaining the parallel decoding benefits.

Importantly, the proposed mask requires no additional training and can be directly applied to existing dLLM decoding pipelines. Since we only modify the design of attention mask and copy few hidden states, our method can be flexibly integrated with other acceleration techniques, such as KVCache and blockwise decoding.
To verify it, we conduct extensive experiments on SDAR~\citep{cheng2025sdar} family dLLMs and four benchmarks, GSM8K~\citep{cobbe2021trainingverifierssolvemath}, MBPP~\citep{austin2021program}, TriviaQA~\citep{joshi-etal-2017-triviaqa}, and MMLU~\citep{hendrycks2020measuring}. Experimental results have demonstrated that our method can achieve up to \(7.46\times\) higher decode throughput, and the generation quality does not degrade and even slightly boosts (+1.7\%), compared with the Vanilla SDAR baseline with tensor parallelism.

%compared with Vanilla decoding (\(+1.7\%\) for both \(B=4\) and \(B=8\)).

%We evaluate our method on the in a training-free setting. 
%We use SDAR-1.7B-Chat as the draft model and SDAR-8B-Chat as the target model, and test block lengths \(B \in \{4,8\}\). 
%Across , our method 
%This shows that the speedup comes from more efficient target verification with the Token-Level Temporal Causal Mask. 

%Large language models (LLMs)~\citep{chowdhery2022palmscalinglanguagemodeling, hurst2024gpt, comanici2025gemini} have achieved remarkable success across a wide range of natural language processing tasks~\citep{zhao2023survey, minaee2024large}. These advances are largely driven by autoregressive (AR) Transformer architectures~\citep{vaswani2017attention}. Despite the performance, AR decoding is inherently sequential, which fundamentally limits generation parallelism~\citep{10.5555/3692070.3692631, xia-etal-2024-unlocking}.
%As an alternative, diffusion language models~\citep{NEURIPS2021_958c5305, Diffusion-LM}~(dLLM) generate text through iterative denoising an incomplete sentence with bidirectional attention and parallel token prediction at each step. Compared with AR models, this formulation reduces decoding latency, allows every position to attend to the full context for stronger global coherence, and exposes the number of denoising steps as a tunable trade-off between quality and speed~\citep{li2025surveydiffusionlanguagemodels, zou2023surveydiffusionmodelsnatural}. Recent work on discrete diffusion large language models (dLLMs)~\citep{labs2025mercuryultrafastlanguagemodels, nie2025llada, ye2025dream7b} has begun to narrow the performance gap with AR systems at scale. Commercial dLLMs such as Mercury Coder~\citep{labs2025mercuryultrafastlanguagemodels}, Gemini Diffusion~\citep{gemini_diffusion}, and LLaDA 2.0~\citep{bie2025llada2} claim parity with strong AR baselines~\citep{hurst2024gpt, jambateam2024jamba15hybridtransformermambamodels} while reporting up to $10\times$ faster inference on various benchmarks.

%Recent commercial dLLMs (\eg Mercury Coder~\citep{labs2025mercuryultrafastlanguagemodels}, Gemini Diffusion~\citep{gemini_diffusion}, and LLaDA 2.0~\citep{bie2025llada2}) are narrowing the performance gap with state-of-the-art AR models, achieving up to $10\times$ faster inference on various benchmarks.
%Despite these gains, the original absence of the causal mask in the bidirectional attention of dLLMs introduces challenges on both the training and inference sides. 
%On the inference side, the headline advantage of dLLMs over AR models is the faster inference enabled by parallel decoding. In the AR setting, speculative decoding has emerged as an important technique for accelerating inference~\citep{xia-etal-2024-unlocking}, in which a small draft model proposes multiple candidate tokens that a larger target model then verifies. The verification step itself relies on the causal mask: a single forward pass over the drafted sequence yields the logits at every position, which permits the target model to validate all proposed tokens simultaneously~\citep{xia-etal-2024-unlocking} \citep{leviathan2023fast,chen2023speculative_sampling}.
%Because dLLMs do not use a token-level causal mask, they cannot use one forward pass to check all drafted tokens under the correct context, as AR models do. As a result, standard token-level speculative decoding does not directly apply to dLLM inference.
% On the training side, an AR model can compute a per-token cross-entropy loss over the entire sequence in a single teacher-forcing pass, since the causal mask guarantees that each position predicts its target from the correct preceding context. A dLLM with full attention does not have this property. Since each position can attend to all other positions, the model may directly see the token it is supposed to predict. Therefore, an unmasked token cannot be used as a valid prediction target. Training therefore relies on randomly masking~\citep{sahoo2024simple, nie2025llada}, a subset of positions at each step and treating only the loss on the masked subset as a valid training signal, which both reduces the effective number of supervised tokens and discards the temporal structure that AR objectives exploit. Random masking creates a mismatch in the conditioning context, where the model may attend to future tokens that should not be visible for prediction while masking past tokens that should otherwise provide useful context.




%Several partial remedies for this limitation have been proposed. Block diffusion~\citep{arriola2025block} introduces a block-level causal attention pattern that restores block-wise parallelism during training and has, in turn, given rise to a line of speculative-style decoding methods that exploit the same block-causal structure to accelerate dLLM inference~\citep{christopher2025specdiff, cheng2025sdar, pan2025blockspec, chen2026dflash}. A complementary line of work splits the training data along inference trajectories, so that the temporal structure becomes part of the supervision signal~\citep{wang2025tracerl}. These approaches offer valuable ways to improve dLLM training or inference. However, they do not directly address the gap between dLLMs and AR models that arises from token-level causal masking. In AR models, the causal mask enables dense token-level supervision during training and one-pass verification during speculative decoding. Without an analogous mechanism, dLLMs still cannot obtain valid logits for the same token across multiple temporal steps in a single forward pass, which limits the efficiency of training-time supervision and standard token-level speculative verification. 

%, and dLLMs cannot fully benefit from AR acceleration methods without an analogous mechanism for maintaining temporally valid token-level contexts.
%To address this limitation directly, we propose the \textbf{Token-Level Temporal Causal Mask}. The key idea is to assign token positions to temporal steps and mask attention so that each position can only use information from earlier steps. This gives dLLMs a valid causal context at the token level. 
% On the training side, this mask permits a dLLM to be supervised in an AR style.~\rtc{Add case study / illustration as figure 1} Combined with the duplicated noisy sequence construction of \citet{arriola2025block}, a single forward pass yields logits for every token in the sequence at all corresponding diffusion time steps, matching the efficiency of AR teacher forcing. In a single teacher-forcing pass, the model can compute loss at every token position because each token is predicted only from its valid causal context, without seeing itself or future tokens. This recovers the full per token cross-entropy signal that vanilla dLLM training discards. The mask further carries a complete temporal structure through the sequence, so each position is conditioned on its proper preceding context rather than on an arbitrary random subset. 
%On the inference side, this restored token-level causal structure enables standard token-level speculative decoding for dLLMs. A target dLLM can verify an entire block of drafted tokens in a single forward pass, recovering the same verification step that AR speculative decoding relies on but that the vanilla dLLM formulation cannot perform. Overall, our method gives dLLMs the key verification abilities that causal masking provides in AR models, while retaining the parallel decoding benefits that make dLLMs attractive. Importantly, the proposed mask is plug-and-play and requires no additional training, allowing it to be applied directly to existing dLLM decoding pipelines.
% 你多写几句啊，这个结论太少了 @Junxia ok
%


% At the mechanism level, the aligned RoPE setting reaches a token-level acceptance rate of \(0.902\) on GSM8K, showing that the target model accepts most drafted tokens when they are verified under the token-level temporal causal context.


\input{src/figure/figure1}


==> neurips26_dllm_causal_mask/src/section/2_related_work.tex <==
\section{Related work}

\paragraph{Diffusion Language Models.}
Masked language modeling was first established as a pretraining objective by BERT style bidirectional encoders\citep{devlin2019bert}, which recover a small fraction of held out tokens from their bidirectional context. Subsequent work recast this objective as a continuous time generative process, with DiffusionBERT~\citep{he-etal-2023-diffusionbert} providing an explicit bridge between BERT style masked prediction and absorbing state diffusion. Building on this masked language modeling tradition, discrete diffusion language models~\citep{nie2025llada, yang2025mmada} corrupt a clean sample by replacing a randomly chosen subset of its tokens with the special symbol $\texttt{[MASK]}$, producing a noised sequence. The forward corruption factorizes across all response token positions: each position is independently replaced by $\texttt{[MASK]}$ with a certain probability.
%Building on this masked language modeling tradition, masked diffusion language models~\citep{nie2025llada, yang2025mmada} corrupt a clean sample $z_0$ by replacing a randomly chosen subset of its tokens with the special symbol $\texttt{[MASK]}$, producing a noised sequence $z_t$ indexed by a continuous noise level $t \in [0,1]$. The forward corruption factorizes across the $L$ response positions: each position is independently replaced by $\texttt{[MASK]}$ with probability $t$ and otherwise kept as $z_0^i$,
%\begin{equation}
%  q(z_t^i = \texttt{[MASK]} \mid z_0) = t,
%  \qquad
%  q(z_t^i = z_0^i \mid z_0) = 1-t,
%  \qquad i = 1, \dots, L.
%\end{equation}
The reverse process supports an accelerated parameterization in which several masked positions are recovered jointly within a single transition from high noise level to a lower level, rather than one position at a time.

% Prior work has shown that the training loss for diffusion language models follows from a likelihood based derivation~\citep{shi2024simplified, sahoo2024simple}\citep{zheng2025masked,ou2025absorbing}
% , and the resulting objective coincides with the evidence lower bound on $\log p_\theta(z)$,
% \begin{equation}
%   \begin{aligned}
%     \mathcal{J}_{\text{full}}(z_0, c, \theta)
%     = \int_0^1 \frac{1}{t\,|z_0|}\,
%       \mathbb{E}_{q(z_t \mid z_0)}\!\left[
%         \sum_{i:\,z_t^i = \texttt{[MASK]}}
%         \log p_\theta\!\left(z_0^i \mid z_t, c\right)
%       \right] dt,
%   \end{aligned}
% \end{equation}
% where $c$ denotes the prompt component of the input, $|z_0|$ is the length of the response, and $p_\theta(z_0^i \mid z_t, c)$ is the model's predictive distribution at position $i$ parameterized by $\theta$. 

% We refer to the \textbf{per token supervision density} of a training objective as the fraction of response positions whose loss contributes a gradient on a single forward pass. AR teacher forcing achieves a supervision density of $1$, since every position predicts its target from the causal prefix and therefore contributes a loss term. The MDM objective in equation~(2) instead has expected supervision density equal to the noise level $t$, since the inner sum runs only over positions sampled into the mask and leaves the unmasked majority without a gradient signal.

\paragraph{Blockwise Decoding for dLLMs.}
A complementary line of work adapts pretrained autoregressive checkpoints into diffusion language models, preserving the AR backbone's linguistic competence while enabling parallel decoding~\citep{ye2025dream7b}. A common strategy is to introduce block causal attention, which imposes causal dependencies across coarse-grained blocks while allowing bidirectional denoising within each block. This design has been adopted by recent dLLMs~\citep{ye2025dream7b, gong2025scaling_diffusion_language_models, cheng2025sdar, xie2025dreamcoder}, suggesting that AR pretraining can transfer effectively to masked diffusion objectives when the attention pattern is properly constrained.
Block diffusion models~\citep{arriola2025block, cheng2025sdar} formalize this idea by partitioning the sequence into contiguous fixed-size blocks and replacing full bidirectional attention with block causal attention. During inference, all positions within a block can be denoised jointly, preserving the parallel sampling advantage of diffusion, while dependencies across blocks remain causal. This structure also enables standard KV caching across blocks, avoiding the cache invalidation issues caused by combining bidirectional attention with KV reuse in full attention dLLMs~\citep{hu2025acceleratingdiffusionlanguagemodel, liu2025dllmcache, ma2025dkvcachecachediffusionlanguage, arriola2025block, wu2025fastdllm}.

%A complementary line of work adapts pretrained autoregressive checkpoints into diffusion language models, preserving much of the AR backbone's linguistic competence while transferring it to a parallel decoding regime~\citep{ye2025dream7b}. Block causal attention provides one way to better exploit this pretrained AR structure, as it maintains causal dependencies across coarse sequence units while permitting bidirectional denoising within each unit. Several recent dLLMs have adopted this recipe and obtained strong downstream performance~\citep{ye2025dream7b, gong2025scaling_diffusion_language_models, cheng2025sdar}\citep{xie2025dreamcoder}, suggesting that the AR pretraining signal transfers gracefully to the masked diffusion objective once the attention pattern is suitably constrained.
%Block diffusion models~\citep{arriola2025block, cheng2025sdar} formalize this transfer by partitioning the sequence into contiguous blocks of fixed size and replacing the bidirectional mask of full attention with block causal attention, an attention pattern that is autoregressive across blocks and bidirectional within each block. 
%On the inference side, block attention preserves the parallel sampling efficiency of diffusion, since all positions inside a block can be denoised jointly while across block dependencies remain causal. A practical consequence is that block causal attention supports a standard KV cache across blocks, avoiding the cache invalidation issues that arise when bidirectional attention is combined with KV reuse in full attention dLLMs~\citep{hu2025acceleratingdiffusionlanguagemodel, liu2025dllmcache, ma2025dkvcachecachediffusionlanguage, arriola2025block, wu2025fastdllm}.
%Concretely, block causal attention assigns to each position $i$ in block $b$ visibility over every position in blocks $1, \dots, b-1$ together with all positions inside block $b$, while positions in later blocks are masked out, where $b \in \{1, \dots, L/B\}$ indexes the $L/B$ blocks of a response of length $L$. 
% The training objective in equation~(2) then factorizes over blocks,
% \begin{equation}
%   \begin{aligned}
%     \mathcal{J}_{\text{block}}(z_0, c, \theta)
%     = \sum_{b=1}^{L/B} \int_0^1 \frac{1}{t\,B}\,
%       \mathbb{E}_{q(z_t^{(b)} \mid z_0^{(b)})}\!\left[
%         \sum_{i:\,z_t^{i,(b)} = \texttt{[MASK]}}
%         \log p_\theta\!\left(z_0^{i,(b)} \mid z_t^{(b)}, z_0^{(<b)}, c\right)
%       \right] dt,
%   \end{aligned}
% \end{equation}
% where $z_0^{(b)}$ and $z_t^{(b)}$ denote the clean and noised tokens inside block $b$, and $z_0^{(<b)}$ denotes the already decoded tokens in earlier blocks.
% On the training side, block causal attention recovers an AR style parallelism property by duplicating the input into a clean copy and a noised copy, so the per-block losses across all $L/B$ blocks can be computed in a single forward pass over roughly $2L$ tokens~\citep{arriola2025block}. This single pass replaces the $L/B$ sequential block level passes that a strict autoregressive treatment of block diffusion would otherwise require, while preserving more supervision per example than fully bidirectional vanilla MDM training. \textcolor{red}{\textbf{[TODO: consider adding a schematic figure here illustrating the duplicated clean/noised input and the cross-copy block causal attention mask.]}} 


% =============================================================================
% 本章节sp的story line
% 第一段 介绍SD的诞生是因为可以在GPU low batch size 提升LLM的推理速度，介绍一下加速的原理
% 第二段 介绍为什么直接将SD迁移到dLLM上是不可行的(block wise 之间的token互相不可见)，而我们提出的new causal mask很好的解决了这个问题
% 第三段 对比已有的dLLM SD的工作，我们是真正意义上SD的范式，并且是training free的，具有更好的迁移性以及更低的部署成本
% =============================================================================

\paragraph{Speculative Decoding.}
Speculative decoding (SD) accelerates LLM inference by using a small draft model to propose multiple candidate tokens and a larger target model to verify them in parallel~\citep{leviathan2023fast, chen2023speculative_sampling}. This paradigm is particularly effective at low batch sizes on GPUs, where decoding is often memory bandwidth bound rather than compute bound. 
%In a typical SD step, the target model performs one forward pass over the drafted block, and a rejection sampling rule accepts the longest valid prefix while preserving the target model's output distribution. 
Subsequent work improves this pipeline through better proposal models, tree-based verification, multi-token prediction heads, feature level drafting, and drafter-free parallel decoding~\citep{miao2023specinfer, cai2024medusa, li2024eagle, fu2024lookahead_decoding}. 
%These methods fundamentally rely on the token-level causal mask in AR models, where each verified token conditions only on previously accepted tokens.
%Directly porting SD to diffusion large language models (dLLMs) breaks this verification step. Since dLLMs do not impose a token-level causal mask along the decoding order~\citep{nie2025llada, ye2025dream7b, gong2025scaling_diffusion_language_models}.
Existing work on diffusion-based speculative decoding falls into two main directions. The first uses diffusion models as drafters for autoregressive verifiers. SpecDiff and SpecDiff-2 train or align diffusion drafters to improve proposal quality for AR targets~\citep{christopher2025specdiff, sandler2025specdiff2}; DiffuSpec instead reuses a pretrained diffusion language model as a training-free drafter while retaining an AR verifier~\citep{li2025diffuspec}, and DFlash explores block diffusion drafting under the same AR target setting~\citep{chen2026dflash}. 
%Public descriptions of DiffuSpec similarly characterize it as using a pretrained diffusion language model for drafting while remaining compatible with standard AR verifiers, which supports this distinction.
The second direction accelerates a single dLLM through self-speculation or trajectory-level verification, where the same diffusion model or block diffusion process proposes and checks candidate states~\citep{gao2025ssd, han2026s2d2, agrawal2025spiffy, pan2025blockspec}. For example, S2D2 is described as a training-free self-speculative decoding framework for block-diffusion language models, where the same pretrained model serves as both drafter and verifier under different modes; BlockSpec similarly targets blockwise speculative decoding for dLLMs by exploring future decoding trajectories. 
%Complementary system-level work focuses on cache reuse, adaptive parallel decoding, and serving efficiency~\citep{wu2025fastdllm, liu2025dllmcache, israel2025apd, wu2026fastdllmv2, liang2026focus, ma2025dinferefficientinferenceframework, fan2025dllmserve, cheng2025sdar}. 
%In contrast, we study cross-model dLLM-to-dLLM speculative decoding, where a smaller pretrained diffusion model drafts tokens and a larger pretrained diffusion model verifies them. The proposed token-level temporal causal mask enables this verification step in a training-free manner, without jointly designing or retraining the drafter and verifier.

%Speculative decoding (SD) accelerates LLM inference by using a small draft model to propose tokens and a larger target model to verify them \citep{leviathan2023fast, chen2023speculative_sampling}. This is especially effective at low batch size on GPUs, where decoding is often limited by memory bandwidth rather than compute. In a typical SD step, the draft model proposes a block of candidate tokens, and the target model checks the whole block in one parallel forward pass. A rejection sampling rule then accepts the longest valid prefix, ensuring that the accepted tokens follow the same distribution as tokens generated directly by the target model. Later work improves different parts of this pipeline, including the proposal model, tree-based verification, multi-token prediction heads, feature-level drafting, and drafter-free parallel decoding \citep{miao2023specinfer, cai2024medusa, li2024eagle, fu2024lookahead_decoding}. These methods all rely on the causal mask of autoregressive models, where each verified token conditions on all previously accepted tokens through causal attention.
%Porting this paradigm directly to diffusion large language models (dLLMs) breaks the verification step. Because dLLMs do not place a token-level causal mask along the decoding order \citep{nie2025llada, ye2025dream7b, gong2025scaling_diffusion_language_models}, a single forward pass over a block of drafted tokens does not yield the per-position conditional distributions that SD rejection sampling requires. The SD rule expects, at each drafted position $k$, the distribution over the $k$-th token given only the previously accepted tokens. A bidirectional dLLM target instead conditions every position on the entire block, so the per-position distributions it produces no longer match the conditionals the rejection rule assumes. The standard token-level SD pipeline therefore does not directly transfer to dLLM inference. Our work resolves this obstacle by equipping the target dLLM with the Token-Level Temporal Causal Mask.
%Existing work that combines diffusion models with speculative decoding can be grouped into two main directions, neither of which addresses the cross-model dLLM-to-dLLM setting studied here. One direction uses diffusion models as drafters for autoregressive verifiers. SpecDiff and SpecDiff-2 train or align a diffusion drafter to improve proposal quality for an AR target \citep{christopher2025specdiff, sandler2025specdiff2}. DiffuSpec reuses a pretrained diffusion language model as a training-free drafter while keeping the verifier autoregressive \citep{li2025diffuspec}, and DFlash explores block diffusion drafting under the same AR-target setting \citep{chen2026dflash}. A second direction accelerates a single dLLM through self-speculation or trajectory-level verification, where the same diffusion model or block diffusion process both proposes and checks candidate states \citep{gao2025ssd, han2026s2d2, agrawal2025spiffy, pan2025blockspec}. These methods avoid maintaining a separate drafter, but they do not consider the setting where a smaller pretrained diffusion model drafts tokens and a larger pretrained diffusion model verifies them. Complementary system-level work on dLLM inference focuses on cache reuse, adaptive parallel decoding, and serving efficiency \citep{wu2025fastdllm, liu2025dllmcache, israel2025apd, wu2026fastdllmv2, liang2026focus, ma2025dinferefficientinferenceframework, fan2025dllmserve, cheng2025sdar}, leaving the cross-model dLLM-to-dLLM speculative decoding problem open. We study this setting directly: both the drafter and verifier are pretrained diffusion language models, and the verification step is enabled by our token-level temporal causal mask. The resulting procedure is training-free and can be applied without jointly designing or retraining the drafter and verifier.


==> neurips26_dllm_causal_mask/src/section/3_methodology.tex <==
\section{Methodology}

% % Setup subsection commented out per user request; revive by removing the iffalse/fi wrapper.
% \iffalse
% \subsection{Setup}

% We adopt the notation of \S2.1 and \S2.2 and work in the block diffusion regime with block size $B$. A response of length $L$ is decoded in $L/B$ steps, each recovering a contiguous block of $B$ tokens.

% The block diffusion training objective $\mathcal{J}_{\text{block}}$ defined in \S2.2 is optimized via the duplicated input scheme of \citet{arriola2025block}, which evaluates the per block losses across all $L/B$ blocks in a single forward pass over roughly $2L$ tokens. Attention is causal across blocks and bidirectional within each block, and inside any single block the training signal is restricted to a random subset of $B$ positions drawn from the corruption distribution. The causal structure therefore lives at the granularity of blocks rather than individual tokens. The per token supervision density inside a block matches vanilla masked diffusion training rather than autoregressive teacher forcing, since only the randomly masked positions contribute gradient on a given pass.

% We push the duplicated input construction down to the granularity of individual decoding steps. The block level causal attention pattern is replaced by a token level temporal causal mask that imposes a strict temporal ordering on the $L$ response positions, so that a single forward pass supervises every response token under its proper temporal causal context. This recovers the per token supervision density of autoregressive teacher forcing on the training side while preserving the parallel sampling behavior of dLLMs at inference. The remainder of this section formalizes the construction via per token temporal labels (\S3.2), specifies the matching position encoding modification (\S3.3), and gives the training procedure and loss (\S3.4).
% \fi
As dLLMs can not maintain temporally valid token-level contexts as AR models to support multiple possible tokens verification in a single forward pass, we aim to devise a new attention masking strategy to solve it in dLLMs.
Based on it, we propose a simple but effective speculative decoding method for accelerating dLLMs during inference, which can significant reduce the inference latency and support the integration with other techniques such as blockwise decoding and KV cache.


\subsection{Token-level Temporal Causal Attention}
\label{sec:Draft model}
%Original dLLMs are based on bidirectional attention to control the visible context. Here, we design token-level temporal causal attention strategy to replace it, to guarantee that each token can attend to its current step context and also other information from the additional reference context. Concretely, we first prepare the input layout that needs to keep the copy of related tokens in the context as reference, then create the attention mask with the consideration of token-level temporal information, and finally predict the masked tokens.
Original dLLMs use bidirectional attention to control the visible context. Here, we replace this design with a token-level temporal causal attention strategy, which ensures that each token can attend to its current step context as well as additional reference information from earlier temporal steps. Concretely, we first construct an input layout that keeps copies of related tokens as reference context, then build an attention mask according to token-level temporal order, and finally align position encodings before predicting the masked tokens.


\paragraph{Input Layout Prepare.}
Given a prompt $c$, we construct the attention context by appending two response sections of length $B$: a data section $D=(D_1,\dots,D_B)$ and a mask section $\widetilde{D}=(\widetilde{D}_1,\dots,\widetilde{D}_B)$. The data section stores reference tokens, while the mask section contains the prediction slots, where $\widetilde{D}_k=\texttt{[MASK]}$. Each pair $(D_k,\widetilde{D}_k)$ corresponds to the same response position but plays different roles: $D_k$ provides contextual information from a reference or previously decoded trajectory, whereas $\widetilde{D}_k$ is the position where logits are computed for token prediction. This layout allows the model to explicitly keep reference tokens in the context while still performing masked token prediction.

%We construct the attention context as the prompt $c$ followed by two response sections of length $B$. The clean data section $D = (D_1, \dots, D_B)$ stores the response tokens that the multi-step ground truth process would have produced, with $D_k$ the token at decoding step $k$. The mask section $\widetilde{D} = (\widetilde{D}_1, \dots, \widetilde{D}_B)$ contains paired placeholder slots, with $\widetilde{D}_k = \texttt{[MASK]}$. By construction, $D_k$ and $\widetilde{D}_k$ refer to the same response token under two roles: the data section supplies the conditioning context that an iterative denoising step would observe, while the mask section identifies the positions on which prediction losses are computed. Depending on the temporal order, tokens in the mask section may also serve as context for later predictions.

%We construct the per-block attention context as the prompt $c$ followed by two response sections of length $B$. The clean data section $D = (D_1, \dots, D_B)$ stores the response tokens that the multi-step ground truth process would have produced, with $D_k$ the token at decoding step $k$. The mask section $\widetilde{D} = (\widetilde{D}_1, \dots, \widetilde{D}_B)$ contains paired placeholder slots, with $\widetilde{D}_k = \texttt{[MASK]}$. By construction, $D_k$ and $\widetilde{D}_k$ refer to the same response token under two roles: the data section supplies the conditioning context that an iterative denoising step would observe, while the mask section identifies the positions on which prediction losses are computed. Depending on the temporal order, tokens in the mask section may also serve as context for later predictions.

\paragraph{Temporal Attention Mask.}
Each response position is assigned a temporal step label \(\tau \in \{1,\dots,B\}\), indicating the inference step associated with that token. We represent this assignment using a step map \(\mu=(\mu_1,\dots,\mu_B)\), a permutation of \(\{1,\dots,B\}\), where both \(D_k\) and \(\widetilde{D}_k\) share the same temporal label \(\tau=\mu_k\). Prompt tokens are assigned \(\tau=0\). For example, the left-to-right order corresponds to \(\mu=(1,2,\dots,B)\), while other permutations allow different decoding orders. This step map extends block-level causal attention~\citep{arriola2025block} to a finer token-level temporal structure within each block.
We define the attention mask \(A\) by \(A_{ij}=1\) if position \(i\) is allowed to attend to position \(j\), and \(A_{ij}=0\) otherwise. Prompt tokens are visible to all response positions. For response positions, the mask is defined as
\begin{equation}
\small
A_{ij} =
\begin{cases}
1 & \text{if } i,j \in D \text{ and } \tau(j) \le \tau(i), \\
1 & \text{if } i \in D,\, j \in \widetilde{D} \text{ and } \tau(j) > \tau(i), \\
1 & \text{if } i \in \widetilde{D},\, j \in D \text{ and } \tau(j) < \tau(i), \\
1 & \text{if } i,j \in \widetilde{D} \text{ and } \tau(j) \ge \tau(i), \\
0 & \text{otherwise.}
\end{cases}
\end{equation}
This mask enforces a temporally valid visible context. A masked prediction slot \(\widetilde{D}_i\) can attend to decoded or reference data tokens from earlier steps, \(D_j\) with \(\tau(j)<\tau(i)\), while future or current unresolved positions remain represented by mask placeholders. Conversely, a data token \(D_i\) is computed from the information that would have been available when it became known: earlier data tokens and later mask placeholders. Padding positions are masked out by zeroing their corresponding rows and columns.

\paragraph{Position Encoding Alignment.}
Because the data and mask sections contain paired positions, their positional encodings must be aligned. Under the above layout, \(D_k\) and \(\widetilde{D}_k\) refer to the same response position but appear at different absolute sequence indices. With standard rotary position embedding (RoPE)~\citep{su2021roformer}, this would rotate their query and key vectors using different position indices, even though they correspond to the same token position. To avoid this mismatch, we apply a RoPE copy strategy: each mask position \(\widetilde{D}_k\) reuses the RoPE index of its paired data position \(D_k\), while prompt and data tokens keep their original absolute indices. This alignment ensures that logits computed at masked positions are positionally consistent with the corresponding response tokens.

\paragraph{Masked Token Prediction.}
After applying the temporal attention mask and position encoding alignment, the model predicts tokens only at the mask section. For a prediction slot \(\widetilde{D}_i\), the visible context consists of the prompt, earlier data tokens \(D_j\) with \(\tau(j)<\tau(i)\), and mask placeholders \(\widetilde{D}_j\) with \(\tau(j)\ge\tau(i)\). Therefore, the logits at \(\widetilde{D}_i\) approximate the token distribution under a temporally consistent context, analogous to the prefix-conditioned distribution used in autoregressive speculative verification. This enables dLLMs to verify drafted tokens at the token level while preserving their parallel decoding structure.
%\paragraph{Attention Mask Creation.}
%Each response position carries a temporal step label $\tau \in \{1, \dots, B\}$ that identifies which iterative denoising step would have generated that token. We pass this label to the model through a step map $\mu = (\mu_1, \dots, \mu_B)$, a permutation of $\{1, \dots, B\}$ that assigns block index $k$ to step $\mu_k$. The data and mask sections share the same step map by index pairing: $D_k$ and $\widetilde{D}_k$ both carry $\tau = \mu_k$. Prompt positions carry $\tau = 0$. For example, the left-to-right map $\mu = (1, 2, \dots, B)$ assigns step $k$ to the $k$-th block position, but any permutation of $\{1, \dots, B\}$ is admissible. The step map refines the coarse block-level structure of \citet{arriola2025block}, in which attention is causal across blocks and bidirectional within each block, into a fine-grained per-token causal structure within a block. Figure~\ref{fig:standard-vs-causal} illustrates this construction.

%The attention mask $A$ is defined by $A_{ij} = 1$ iff position $i$ may attend to position $j$. Prompt positions are fully visible to and from every response position. Among the response positions,
%\begin{equation}
%A_{ij} =
%\begin{cases}
%1 & \text{if $i,j \in D$ and $\tau(j) \le \tau(i)$,} \\
%1 & \text{if $i \in D$, $j \in \widetilde{D}$, and $\tau(j) > \tau(i)$,} \\
%1 & \text{if $i \in \widetilde{D}$, $j \in D$, and $\tau(j) < \tau(i)$,} \\
%1 & \text{if $i,j \in \widetilde{D}$ and $\tau(j) \ge \tau(i)$,} \\
%0 & \text{otherwise.}
%\end{cases}
%\end{equation}

%The four response-side cases have a clean structural reading. The data--data block is the standard $B \times B$ autoregressive causal mask ($\tau(j) \le \tau(i)$), and the mask--mask block is its reverse causal counterpart ($\tau(j) \ge \tau(i)$). The two cross blocks complement these along strict inequalities: data attends to later mask positions ($\tau(j) > \tau(i)$), and mask attends to earlier data positions ($\tau(j) < \tau(i)$). Padding positions are masked out symmetrically by zeroing their rows and columns.


%\subsection{Position Encoding Alignment}
%Rotary position embedding rotates the query and key vectors by an angle that depends on the absolute sequence index \citep{su2021roformer}. Under the layout of \S3.1, the $k$-th data position sits at absolute index $|c| + k$ while its paired mask position sits at $|c| + B + k$; the standard rule would therefore rotate them at different frequencies even though they refer to the same response token at decoding step $k$.
%We resolve this by a RoPE copy: when computing the rotary embedding, each mask position is indexed at the absolute position of its paired data position. The prompt and data sections keep their own absolute indices, while every mask position simply reuses the RoPE values of its paired data slot. With this alignment, the rotated query and key vectors at every mask position match what the model would have produced for the corresponding response token at its own decoding step. Without it, the attention construction of \S3.1 would no longer faithfully simulate iterative denoising.

%\paragraph{Masked Token Prediction.}
%The mask section specifies what information is available when predicting a token at temporal step $\tau(i)$. At this step, tokens with smaller temporal labels have already been decoded and can be used as context, while tokens with labels greater than or equal to $\tau(i)$ are still represented by mask placeholders. Therefore, the query at $\widetilde{D}_{\tau(i)}$ attends to the prompt, to decoded data positions $D_{\tau(j)}$ with $\tau(j) < \tau(i)$, and to placeholder positions $\widetilde{D}_{\tau(j)}$ with $\tau(j) \ge \tau(i)$.
%The data section plays a complementary role. Once a token $D_{\tau(i)}$ is decoded, later temporal steps will use it as conditioning context. Its representation should therefore be computed from the information that would have been available when that token first became known. We implement this by allowing $D_{\tau(i)}$ to attend to data positions with temporal labels at most $\tau(i)$, and to mask placeholders with labels strictly greater than $\tau(i)$. This makes the hidden state of $D_{\tau(i)}$ consistent with its role as an already-decoded context token for later predictions.


\input{src/figure/figure2}

% \subsection{Aligned position encoding via RoPE copy}

% \paragraph{Positional mismatch.}
% Rotary position embedding rotates the query and key vectors at each position by an angle that depends on that position's absolute sequence index \citep{su2021roformer}. Under the input layout of \S3.1, the $k$-th data position sits at absolute index $|c| + k$ while the $k$-th mask position sits at absolute index $|c| + B + k$, so the standard rule would assign the two positions different rotational frequencies. The two positions, however, refer to the same response token at decoding step $k$, and the mask placeholder must therefore behave as if it occupied the same sequence position as its paired data token.

% \paragraph{Logical position remapping.}
% We capture this requirement through a logical position map $\pi : \{1, \dots, N\} \to \mathbb{Z}_{\ge 0}$ that overrides the absolute index used by the rotary embedding,
% \begin{equation}
% \pi(i) =
% \begin{cases}
% i & \text{if $\sigma(i) \in \{\textsf{C}, \textsf{D}\}$,} \\
% i - B & \text{if $\sigma(i) = \widetilde{\textsf{D}}$.}
% \end{cases}
% \end{equation}
% The map is the identity on the prompt and data sections and shifts each mask position back by $B$ slots. In particular, $\pi(|c| + B + k) = |c| + k$, so the $k$-th mask position is assigned the same logical index as its paired data position. We refer to $\pi$ as a remap rather than a permutation, since the image of the mask section coincides with the image of the data section by design.

% \paragraph{RoPE copy implementation.}
% Concretely, RoPE is applied using the logical position $\pi(i)$ rather than the absolute position $i$, so the cosine and sine tables are indexed by $\pi(i)$. Because $\pi$ leaves the prompt and data sections unchanged and maps each mask position to its paired data position, this amounts to directly reusing the data section's RoPE values for the corresponding mask positions.

% \paragraph{Aligned RoPE geometry.}
% % \paragraph{Position alignment.}
% Without this remap, each mask placeholder would carry the rotation of a token at absolute index $|c| + B + k$ rather than the rotation of the response token at step $k$ that it represents, and the attention construction of \S3.1 would no longer faithfully simulate iterative denoising. With the remap, the geometry of the rotated query and key vectors at every mask position matches what the model would have produced for the corresponding response token at its own decoding step.


% \subsection{Application for Training}

% The construction of \S3.1 and \S3.2 yields a per-block training objective that can be computed in a single forward pass. Given a clean response $z_0$ and prompt $c$, we form the input $X = c \,\Vert\, D \,\Vert\, \widetilde{D}$ of length $N = |c| + 2B$, where $D_k$ is the $k$-th response token and $\widetilde{D}_k$ is its paired mask placeholder. 
% % This duplicated layout increases the response-block portion of the input from $B$ to $2B$ tokens. However, this overhead is not unique to our method: block-causal training baselines based on duplicated clean/noised blocks use the same block-level sequence length. Thus, our comparison to block-causal attention is made under a matched input-length setting.

% We then run the model under the attention mask $A$ and position remap $\pi$. The output projection followed by softmax produces a categorical distribution $p_\theta(\,\cdot\, \mid X, A, \pi)$ at every position. For step $k$, we use the distribution at the paired mask position $|c| + B + k$, whose attention context matches the information available to an iterative denoising step at temporal index $k$. We supervise this distribution against the corresponding data token $D_k$. The per-block training objective is
% \begin{equation}
% \mathcal{J}_{\text{tok}}(z_0, c, \theta) = \frac{1}{B} \sum_{k=1}^{B} \log p_\theta\!\left(D_k \,\big|\, X, A, \pi, \; \text{position } |c| + B + k\right),
% \end{equation}
% We train by maximizing $\mathcal{J}_{\text{tok}}$, defined with notation consistent with the $\mathcal{J}_{\text{full}}$ and $\mathcal{J}_{\text{block}}$ objectives in \S2.1 and \S2.2. Prompt and data positions act as conditioning context and contribute no direct loss term, although they receive gradients through attention.

% The main training-side advantage over block diffusion is higher supervision density. In block diffusion, each forward pass uses a randomly noised block, and the loss is computed only on the positions selected as masked in that sample. As a result, only a subset of the $B$ positions inside the block receives direct gradient on a given pass. In contrast, our token-level objective creates a prediction slot for every position in the block and supervises all $B$ positions in the same forward pass. It therefore matches the per-token supervision density of autoregressive teacher forcing while preserving parallel sampling at inference.

% The forward pass is performed on $N = |c| + 2B$ tokens rather than on the $|c| + B$ tokens used by a single-view per-block computation, so the duplicated layout adds $B$ tokens of overhead per block. Aggregated across all $L/B$ blocks of a response, the full forward pass operates on roughly $|c| + 2L$ tokens. This matches the sequence-length scale of the duplicated clean/noised input used in the block diffusion training scheme of \citet{arriola2025block}, while replacing block-level causality with token-level temporal causality. This cost should be compared with a strict step-by-step replay of the iterative denoising process, which would require $B$ sequential forward passes for a block of size $B$. In contrast, our training procedure obtains the losses for all $B$ temporal steps in one forward pass. This one-pass computation is the main efficiency advantage of the proposed training procedure (see §X.X for empirical validation).~\rtc{We may refer to some experiment results as evidence.}

% A response of length $L$ partitions into $L/B$ blocks under the regime of \S3.1, and our training procedure applies the per block construction to every block of the response inside a single forward pass. Concretely, each block $b \in \{1, \dots, L/B\}$ contributes its own data section $D^{(b)}$ and mask section $\widetilde{D}^{(b)}$, and the input is the concatenation of the prompt followed by the data and mask sections of all blocks. The attention mask is causal across blocks, so positions in block $b$ may attend to clean tokens of blocks $1, \dots, b-1$ but not to later blocks, and within each block the per token rules of \S3.1 are applied unchanged. The full training objective is the mean of the per block objectives $\mathcal{J}_{\text{tok}}^{(b)}$ across all $L/B$ blocks of the response.

% The construction is an approximation rather than an exact replay of sequential decoding, as discussed at the end of \S3.1. The gap arises from evaluating all hidden states in parallel within a single forward pass, which neglects higher-order dependencies (e.g., second-order attention effects between intermediate states). Prior work suggests that such higher-order effects introduce negligible error in practice; combined with our empirical results, this indicates that the approximation is effectively near-exact.

\subsection{Application for Speculative Decoding}
\label{sec:speculative-decoding}
%We next describe how the token-level temporal causal attention strategy enables standard speculative decoding in dLLMs. First, a smaller dLLM plays the role of the draft model to collect the candidate tokens and their orders. Then, we use the target model to score all candidate for verifying their acceptance.

We next describe how token-level temporal causal attention enables standard speculative decoding for dLLMs. Speculative decoding typically uses a small draft model to propose candidate tokens and a larger target model to verify them in parallel with rejection sampling~\citep{leviathan2023fast, chen2023speculative_sampling}. In our setting, both the drafter and verifier are dLLMs: the smaller dLLM first proposes candidate tokens together with their temporal order, and the target dLLM then scores all candidates in a single forward pass using the proposed token-level temporal causal mask.


% \paragraph{Drafting.}
% We next describe how the token-level temporal causal mask enables standard token-level speculative decoding with a diffusion target model. Consider a dLLM decoding block of length $B$, and let $R$ denote the number of remaining undecoded positions in the current block. When $R \ge \gamma$, a smaller draft dLLM with parameters $\phi$ proposes $\gamma$ candidate tokens for a subset of the remaining positions,
% \[
% \widehat{D} = (\widehat{D}_{o_1},\ldots,\widehat{D}_{o_\gamma}),
% \]
% where $o_1,\ldots,o_\gamma$ denotes the draft-induced temporal order. During this draft process, the drafter determines both the candidate tokens and the temporal order in which they are produced. We denote the corresponding draft-induced step map by
% \[
% \mu^\phi_{o_r}=r,\qquad r=1,\ldots,\gamma.
% \]
% The target verifier uses this same step map to check the drafted tokens.

\paragraph{Draft Model for Candidates Collection.}

Consider a dLLM decoding sequence of length $B$, and let $R$ denote the number of remaining undecoded positions. When $R \ge \gamma$, a smaller draft dLLM with parameters $\phi$ proposes $\gamma$ candidate tokens $\widehat{D} = (\widehat{D}_{o_1}, \ldots, \widehat{D}_{o_\gamma})$, where $o_1,\ldots,o_\gamma$ denotes the draft-induced temporal order. Specifically, position $o_r$ is generated at draft step $r$. The drafter therefore determines both the candidate tokens and the order in which they should be verified. The target verifier reuses this order by assigning temporal label $\tau=r$ to the slot corresponding to $\widehat{D}_{o_r}$.

\paragraph{Target Model Verification.}
The verification input follows the paired data-mask layout introduced in Sec.~\ref{sec:Draft model}, but only for the $\gamma$ drafted positions in the current speculative step. The $r$-th data slot stores the drafted token $\widehat{D}_{o_r}$, and the paired mask slot serves as its verification position. We then construct the temporal attention mask using $\tau=r$ for each drafted token and apply the same RoPE-copy alignment between each drafted token and its paired verification slot.
Under this mask, the verification slot for $\widehat{D}_{o_r}$ can attend to the prompt and to earlier drafted tokens $\widehat{D}_{o_1},\ldots,\widehat{D}_{o_{r-1}}$, but not to the current token or later drafted tokens. Thus, the target distribution at this slot, denoted by $p_\theta^{(r)}$, scores $\widehat{D}_{o_r}$ under the valid draft-induced causal context. Importantly, all target distributions $\{p_\theta^{(r)}\}_{r=1}^{\gamma}$ are obtained from one target forward pass, allowing the target dLLM to verify multiple drafted tokens in parallel while preserving token-level causal validity.
We apply the standard speculative decoding acceptance rule along the draft-induced temporal order. Let $p_\phi^{(r)}$ be the draft distribution used to sample $\widehat{D}_{o_r}$. For $r=1,\ldots,\gamma$, the candidate token is accepted with probability
\begin{equation}
\small
\alpha_r
=
\min\left(
1,
\frac{
p_{\theta}^{(r)}(\widehat{D}_{o_r})
}{
p_{\phi}^{(r)}(\widehat{D}_{o_r})
}
\right).
\end{equation}
The algorithm accepts the longest prefix before the first rejection. If $\widehat{D}_{o_r}$ is rejected, the remaining drafted suffix is discarded, and the target dLLM  samples the token at position $o_r$. The next speculative step then continues from the updated block state. If all $\gamma$ candidates are accepted, they are committed to the block, and speculative decoding proceeds while at least $\gamma$ undecoded positions remain. When fewer than $\gamma$ positions remain, drafting stops and the target dLLM completes the block directly.

\paragraph{Training-free Deployment.}
The proposed procedure is training-free. It only modifies the verification-time input layout, attention mask, and RoPE indexing, and can therefore be applied to pretrained draft and target dLLMs without parameter updates. The rejection-sampling correction preserves the target distribution induced by the token-level temporal causal mask, while reducing the number of expensive target forward passes. This makes cross model dLLM-to-dLLM speculative decoding practical without jointly designing or retraining the drafter and verifier.

%Consider a dLLM decoding block of length $B$, and let $R$ denote the number of remaining undecoded positions in the current block. When $R \ge \gamma$, a smaller draft dLLM with parameters $\phi$ proposes $\gamma$ candidate tokens $\widehat{D} = (\widehat{D}_{o_1},\ldots,\widehat{D}_{o_\gamma})$ for a subset of the remaining positions, where $o_1,\ldots,o_\gamma$ is the draft-induced temporal order: position $o_r$ is generated at draft step $r$. The drafter determines both the candidate tokens and this order, and the target verifier reuses the same order-equivalently, sets $\tau = r$ at the slots of $\widehat{D}_{o_r}$---to check the drafted tokens.

% \paragraph{Verification layout.}
% The verification input follows the same data--mask paired layout as in \S3.1, but is applied only to the $\gamma$ drafted positions in the current speculative step:
% \[
% X^{\mathrm{ver}} = c \,\Vert\, \widehat{D} \,\Vert\, \widetilde{D}.
% \]
% The data section contains the drafted tokens ordered by the draft-induced temporal order
% $o_1,\ldots,o_\gamma$, and the mask section contains their paired placeholder positions in the same order. Thus, the $r$-th data position stores $\widehat{D}_{o_r}$, and the $r$-th mask position is its paired verification slot.

% We build the attention mask $A^\phi$ using the draft-induced step map $\mu^\phi_{o_r}=r$. We also use a verification-time RoPE remap $\pi^{\mathrm{ver}}$ that assigns each mask position the same logical position id as its paired data position, following the same principle as \S3.2. This keeps the RoPE geometry aligned between each drafted token and its verification slot. Thus, the verifier does not impose a fixed left-to-right order. Instead, it verifies the candidates in the temporal order proposed by the draft model.

%\paragraph{Verification layout.}

% \paragraph{Target scoring.}
% Under this mask, the paired mask position for the token generated at draft step $r$ can attend to the prompt and to drafted tokens from earlier draft steps, but it cannot attend to the current token or to tokens generated at later draft steps. Let $\mathrm{mask}(o_r)$ denote the paired mask slot of $\widehat{D}_{o_r}$ in the verification input $X^{\mathrm{ver}}$. The target distribution for this token is
% \[
% p_{\theta}^{(r)}(\cdot)
% =
% p_{\theta}\!\left(
% \cdot
% \,\middle|\,
% X^{\mathrm{ver}}, A^\phi, \pi^{\mathrm{ver}},
% \mathrm{position}=\mathrm{mask}(o_r)
% \right).
% \]
% This distribution scores the drafted token $\widehat{D}_{o_r}$ under the same temporal context used by the draft process, namely the prompt and the previously drafted tokens
% \[
% \widehat{D}_{o_1},\ldots,\widehat{D}_{o_{r-1}}.
% \]
% Importantly, all target distributions $\{p_{\theta}^{(r)}\}_{r=1}^{\gamma}$ are obtained from a single target forward pass. This is the key verification behavior we need: the target dLLM checks multiple drafted tokens in parallel, while each token is still scored under its valid draft-induced causal context.

%\paragraph{Verification with Target Model Scoring.}
%The verification input follows the same data--mask paired layout as in \S3.1, but is applied only to the $\gamma$ drafted positions in the current speculative step. The $r$-th data slot stores $\widehat{D}_{o_r}$ and the $r$-th mask slot is its paired verification placeholder. Plugging $\tau = r$ at the slots of $\widehat{D}_{o_r}$ into the construction of \S3.1 yields the verification-time attention mask, and the RoPE copy of \S3.2 keeps the rotary geometry aligned between each drafted token and its verification slot. The verifier therefore does not impose a fixed left-to-right order: it verifies the candidates in the temporal order proposed by the drafter.
%Under this mask, the mask slot paired with $\widehat{D}_{o_r}$ can attend to the prompt and to drafted tokens from earlier draft steps, but not to the current token or to tokens at later draft steps. We write the resulting target distribution at this slot as $p_{\theta}^{(r)}$. By construction, $p_{\theta}^{(r)}$ scores $\widehat{D}_{o_r}$ under the same temporal context used by the drafter---the prompt together with $\widehat{D}_{o_1},\ldots,\widehat{D}_{o_{r-1}}$. All $\gamma$ target distributions $\{p_{\theta}^{(r)}\}_{r=1}^{\gamma}$ are obtained from a single target forward pass: the target dLLM checks multiple drafted tokens in parallel while each token is still scored under its valid draft-induced causal context.
%We then apply the standard speculative decoding acceptance rule along the draft-induced temporal order. Let $p_{\phi}^{(r)}$ denote the draft distribution used to sample $\widehat{D}_{o_r}$ at draft step $r$. For $r=1,\ldots,\gamma$, the candidate token $\widehat{D}_{o_r}$ is accepted with probability
%\[
%\alpha_r
%=
%\min\left(
%1,
%\frac{
%p_{\theta}^{(r)}(\widehat{D}_{o_r})
%}{
%p_{\phi}^{(r)}(\widehat{D}_{o_r})
%}
%\right).
%\]
%The procedure accepts the longest prefix in the draft-induced temporal order before the first rejection. If token $\widehat{D}_{o_r}$ is rejected, the remaining drafted suffix is discarded, and the target dLLM directly generates the token at position $o_r$. The next speculative step then continues from the updated block state. If all $\gamma$ candidates are accepted, the accepted tokens are committed to the current block, and speculative decoding continues while at least $\gamma$ positions remain. When fewer than $\gamma$ positions remain, we stop drafting and let the target dLLM complete the remaining positions directly.

%\paragraph{Training-free deployment.}
%This procedure is training-free. It changes only the verification-time input layout, attention mask, and RoPE indexing, and therefore can be applied to pretrained draft and target dLLMs without modifying their parameters. The resulting target distribution is the temporally factorized distribution induced by the draft-induced token-level causal mask, and the speculative decoding correction above preserves this target distribution while reducing the number of expensive target forward passes.

%\paragraph{Draft-induced causal context.}
%The key difference from vanilla full-attention dLLM verification is the conditioning context used by the target. Without a token-level temporal causal mask, a single target forward pass would not provide the conditional distributions required by token-level speculative decoding. The verifier would either expose each position to too many drafted tokens or fail to condition it on the previously drafted tokens that should already be available. Our mask avoids this issue by using the drafter's own temporal order: the token generated at draft step $r$ is verified using exactly the tokens generated at earlier draft steps as context.


\subsection{Efficiency Discussion} 

Consider one speculative verification step with draft length $\gamma$. Let $T_\theta$ be the walltime of one target dLLM verification pass, and let $T_\phi$ be the average walltime of one draft step. One speculative verification step with draft length $\gamma$ costs, where $\rho$ define the draft-to-target cost ratio:
\begin{equation}
\small
T_{\mathrm{SD}}(\gamma)=\gamma T_\phi + T_\theta=(1+\gamma\rho)T_\theta;~\rho = \frac{T_\phi}{T_\theta}.
\end{equation}
%We provide a simple speedup model for the speculative decoding procedure in \S\ref{sec:speculative-decoding}, 
Following the analysis of \citet{leviathan2023fast}, we aim to quantify the benefit of verifying multiple draft tokens with one target forward pass. Our verification layout introduces an additional overhead because it duplicates the drafted sequence to form the data-mask paired input. Let $\ell$ denote the draft sequence length and let $n$ be the original verification sequence length before duplication. The paired layout increases the effective sequence length from $n$ to $n+\ell$. Therefore, the attention cost increases from $O(n^2)$ to $O((n+\ell)^2)$, with an extra cost. 
\begin{equation}
O((n+\ell)^2 - n^2)
=
O(2n\ell + \ell^2).    
\end{equation}

% Each speculative verification step drafts and verifies at most \(\gamma\) candidate tokens. The acceptance rule is the one defined in \S\ref{sec:speculative-decoding}. We summarize its effect by an average acceptance rate \(\bar{\alpha}\), defined as the mean probability that a drafted token is accepted under the target distributions produced by the one-pass verifier.
% Let $G_\gamma$ denote the number of tokens committed by one speculative verification step with draft length $\gamma$. If the first rejection occurs at draft step $r$, then the first $r-1$ draft tokens are accepted and the target model supplies the corrected token at step $r$, so $G_\gamma=r$. If all $\gamma$ drafted tokens are accepted, then $G_\gamma=\gamma$. Under the i.i.d. acceptance approximation,
% \[
% \Pr(G_\gamma=r) = (1-\bar{\alpha})\bar{\alpha}^{r-1},
% \qquad r=1,\ldots,\gamma-1,
% \]
% and
% \[
% \Pr(G_\gamma=\gamma) = \bar{\alpha}^{\gamma-1}.
% \]
% Therefore, the expected number of committed tokens per target verification pass is
% \[
% \mathbb{E}[G_\gamma]
% =
% \sum_{r=1}^{\gamma-1} r(1-\bar{\alpha})\bar{\alpha}^{r-1}
% +
% \gamma\bar{\alpha}^{\gamma-1}
% =
% \frac{1-\bar{\alpha}^{\gamma}}{1-\bar{\alpha}}.
% \]
% When $\bar{\alpha}=1$, this expression is understood by continuity as $\mathbb{E}[G_\gamma]=\gamma$. This quantity captures the token gain from one-pass verification: when $\bar{\alpha}$ is high, a single target forward pass verifies and commits many drafted tokens; when $\bar{\alpha}$ is low, the procedure approaches target-only decoding.

% If the first rejection occurs at draft step $r$, then $r-1$ drafted tokens are accepted and the target supplies the corrected token at step $r$, committing $r$ tokens total; if all $\gamma$ candidates are accepted, the step commits $\gamma$ tokens. Under the i.i.d. acceptance approximation, the rejection step is geometric with parameter $1-\bar{\alpha}$, so the expected number of committed tokens per target verification pass is
% \[
% \sum_{r=1}^{\gamma-1} r\,(1-\bar{\alpha})\bar{\alpha}^{r-1}
% + \gamma\,\bar{\alpha}^{\gamma-1}
% = \frac{1-\bar{\alpha}^{\gamma}}{1-\bar{\alpha}},
% \]
% which equals $\gamma$ at $\bar{\alpha}=1$ by continuity. When $\bar{\alpha}$ is high, a single target pass commits many drafted tokens; when $\bar{\alpha}$ is low, the procedure approaches target-only decoding.

\paragraph{Adaptation under Blockwise Decoding and KV Cache.}
The duplicated verification layout has a bounded overhead under blockwise decoding with KV cache. 
Let \(n\) be the prefix length and \(\ell\) be the duplicated draft length. 
%Without KV cache, duplicating the verification input increases the attention cost from \(O(n^2)\) to \(O((n+\ell)^2)\). incurring an overhead of
With KV cache, the prefix keys and values are reused, so the verifier only computes the newly introduced duplicated positions. 
Thus the additional computation is bounded by
\begin{equation}
O((n+\ell)^2-n^2)=O(n\ell+\ell^2) \le O(nB+B^2).
\end{equation}
where the inequality follows from \(\ell \le B\) under blockwise decoding. 
Since \(B\) is a small constant in our experiments, e.g., \(B=4\) or \(B=8\), the overhead is effectively linear in the cached prefix length and is much smaller than duplicating and recomputing the full response sequence. In practical settings, this overhead is acceptable.
% This recurrence captures the block-boundary effect that is absent from the standard unbounded analysis of speculative decoding. When many positions remain in the block, one-pass verification improves efficiency by committing multiple draft tokens per target pass. Near the end of a block, however, if fewer than $\gamma$ positions remain, launching another speculative step would be inefficient under the fixed block layout, so the method falls back to target-only completion. The token-level temporal causal mask is what makes each speculative step efficient: it allows the target dLLM to obtain all $\gamma$ conditional distributions in a single forward pass, rather than running one target pass per temporal step.

==> neurips26_dllm_causal_mask/src/section/4_exp.tex <==
\section{Experiments}

\subsection{Experimental setup}

\paragraph{Models.} Following previous studies\citep{leviathan2023fast}\citep{chen2023speculative_sampling}, we use small scale draft model and large scale target model from the same model series for the speculative decoding experiments. We use dLLMs trained with different block lengths from the widely used SDAR\citep{cheng2025sdar} series.

\paragraph{Datasets \& metrics.}
To assess the generation efficiency and effectiveness of our method, we evaluate it on four standard benchmarks covering different task categories: \textbf{GSM8K}~\citep{cobbe2021trainingverifierssolvemath} for mathematical reasoning, \textbf{MBPP}~\citep{austin2021program} for code generation, and \textbf{TriviaQA}~\citep{joshi-etal-2017-triviaqa} and \textbf{MMLU}~\citep{hendrycks2020measuring} for general NLP and knowledge-intensive evaluation. For efficiency, we report \textbf{TPS} and the \textbf{speedup ratio} against vanilla decoding. For effectiveness, we report accuracy for GSM8K, TriviaQA, and MMLU, and pass@1 for MBPP.

\paragraph{Baselines.}
(i) \textbf{Vanilla} follows the standard dLLM decoding procedure with block causal attention and KV cache. Since speculative decoding uses two GPUs, we run Vanilla with tensor parallelism = 2 for a fair comparison. 
(ii) \textbf{Vanilla with CUDA Graph} augments Vanilla decoding with CUDA Graphs to reduce kernel launch overhead. 
(iii) \textbf{S2D2}~\citep{han2026s2d2} performs training free self speculation, where the dLLM first drafts tokens and then verifies them from left to right using the same model with block size set to 1. SSD~\citep{gao2025ssd} is designed for fully bidirectional dLLMs such as LLaDA and Dream, while our experiments use SDAR~\citep{cheng2025sdar}, a block causal dLLM models series with KV cache. BlockSpec~\citep{pan2025blockspec} is orthogonal to our verifier-side contribution, as it focuses on blockwise trajectory speculation rather than token-level target verification. Therefore, these methods are not direct baselines under our SDAR-based setting, and we do not include them in the main comparison.

\paragraph{Configurations.}

We follow the default prompts and chat templates from the OpenCompass~\citep{2023opencompass} evaluation framework. 
Unless otherwise specified, we fix the maximum generation length to \(L=512\) and set the number of denoising steps to the response sequence length \(N\). 
For block length \(B=4\), we use SDAR-1.7B-Chat as the draft model and SDAR-8B-Chat as the target model; for block length \(B=8\), we use SDAR-1.7B-Chat-b8 and SDAR-8B-Chat-b8. 
We set the speculative draft length to \(\gamma=B\), and fall back to vanilla target decoding when the number of remaining positions in the current block satisfies \(R<\gamma\). 
All generation-quality evaluations are conducted in the zero-shot setting with temperature \(=1.0\) and top\_\(p=1.0\). 
All experiments use batch size \(1\), FP32 precision, and KV cache. 
We use two NVIDIA RTX PRO 6000 Blackwell GPUs, with the draft and target models deployed on separate GPUs to avoid resource contention; for the Vanilla baseline, we use tensor parallelism of size \(2\). 
CUDA Graph is enabled for all methods except the basic Vanilla baseline. 
Throughput is measured as decoded tokens per second, excluding prompt prefilling, with \(3\) warmup runs. 
For speed evaluation, we use \(200\) examples from each dataset, while generation quality is evaluated on the full benchmark. 
Speedup is computed relative to Vanilla TP-2 under the same block length.

\subsection{Main results}
\input{src/table/throughput_main_results}
\paragraph{Efficiency Performance.}
Table~\ref{tab:sd_pipe_fast_denoise_tp2_speedup} demonstrates the main efficiency comparison between our method and various baselines. Overall, our method consistently outperforms all the other baselines on decoding throughput across all benchmarks and block sizes. Our method reaches \(71.6\) and \(81.8\) tokens/s on average for \(B=4\) and \(B=8\), corresponding to \(7.46\times\) and \(5.40\times\) speedups over Vanilla decoding. Compared with S2D2, our method also provides substantially higher throughput, showing that our construction of temporal causal mask provides more precise context information.
\input{src/table/eos_bounded_quality_efficiency}
\paragraph{Accuracy performance.}
As the results shown in table~\ref{tab:pass1_sd_vanilla}, it is convinced that our speculative decoding method preserves generation quality comparable to, and in some cases slightly better than, vanilla decoding. Across block lengths 4 and 8, the average performance remains on par with vanilla decoding and even shows small improvements. For block length 4, the average score increases from $0.696$ under vanilla decoding to $0.713$ with speculative decoding. Similarly, for block length 8, the average score improves from $0.681$ to $0.698$. Although our attention mask construction introduces a certain approximation to the exact step by step denoising process, these results indicate that the approximation does not noticeably harm task accuracy in the speculative decoding setting. Instead, the proposed verification mechanism improves decoding efficiency while maintaining, and sometimes slightly improving, generation quality.
\subsection{Additional Results}
\paragraph{Precision Analysis of SimSD.}
Since all positions are evaluated in one forward pass, this construction is not an exact lossless replay of sequential denoising. Instead, it provides an approximation of the same temporal conditioning structure. The approximation arises only from higher order interactions among hidden states that are computed simultaneously, while the direct attention visibility of each position matches the intended denoising step.

We use two experiments to quantify the practical effect of this approximation. (i) \textbf{Self draft distribution analysis.} In this setting, we compare the output distributions induced by conventional generation and by SD generation conditioned on the correct tokens, which directly measures the distributional discrepancy introduced by the parallel construction. (ii) \textbf{Cross model distribution analysis.} In the second experiment, we evaluate whether this approximation affects the normal speculative decoding pipeline, where draft tokens are proposed by a smaller model and verified by a larger target model.

We further analyze the distributional approximation error introduced by the causal mask construction. For both figures, $D$ and $V$ in $\mathrm{KL}(D\|V)$ denote the draft and verification distributions, respectively, and Loss denotes the CE loss. As shown in Figure~\ref{fig:cross_model} and Figure~\ref{fig:self_draft}, the discrepancy between sequential denoising and parallel verification gradually increases from step 0 to step 3. In the self draft setting, $\mathrm{KL}(D\Vert V)$ increases from $0.0889$ at step 0 to $0.2537$ at step 3, while the loss increases from $0.0141$ to $0.2567$. A similar trend appears in the cross model setting, where $\mathrm{KL}(D\Vert V)$ increases from $0.1528$ at step 0 to $0.5010$ at step 3, and the loss increases from $0.0605$ to $0.4389$.

The self draft setting consistently exhibits smaller approximation error than the cross model setting. For example, at step 3, $\mathrm{KL}(D\Vert V)$ is $0.2537$ for self draft but $0.5010$ for cross model, and the corresponding loss is $0.2567$ versus $0.4389$. This is expected because self draft uses the same model on both sides, whereas cross model verification additionally includes the distributional mismatch between the draft and target models. Nevertheless, the overall approximation error remains small in both settings, as reflected by the high top 1 agreement. The self draft setting maintains top 1 agreement of at least $0.9750$, and the cross model setting remains at least $0.9400$ even at the last step. These results indicate that the causal mask provides highly accurate reference context for each verification position, quantitatively explaining why the main accuracy results do not show degradation under our speculative decoding method.
\input{src/figure/figure3_4}
\paragraph{Effect of $\gamma$.}
We analyze how the choice of $\gamma$ affects the quality and efficiency of SimSD. As shown in Table~\ref{tab:gamma_effect_gsm8k}, both the realized acceptance rate and final accuracy generally increase as $\gamma$ becomes larger. This trend suggests that a longer draft scope provides richer target side verification context, allowing SimSD to accept higher quality draft tokens and produce more reliable generations. In particular, increasing $\gamma$ from 3 to 8 improves real $\alpha$ from 0.834 to 0.964 and accuracy from 50.0\% to 82.0\%, showing that larger $\gamma$ values can substantially improve the quality of the draft and verify process.

In contrast, TPS does not exhibit a simple monotonic pattern with respect to $\gamma$. This is expected because changing $\gamma$ affects more than the verification computation itself. A larger $\gamma$ changes the number of tokens verified per step, the interaction between $\gamma$ and the block length, and the overhead of KV cache management during multi block verification. These factors jointly determine the end to end runtime, so the throughput cannot be explained solely by the acceptance rate or the verification scope. For example, $\gamma=4$ achieves the highest TPS in our experiment, while $\gamma=8$ achieves the best accuracy and acceptance rate. This indicates a practical tradeoff: larger $\gamma$ improves generation quality and acceptance behavior, whereas intermediate $\gamma$ values may provide a better speed quality balance. Therefore, we choose $\gamma$ equal to the block length for main experiment, which provides the best overall balance between generation quality and TPS in our setting.

\input{src/table/gamma}

\paragraph{Ablation Study on RoPE Alignment.}
To examine the impact of RoPE alignment, we fix the attention structure and vary only the position ids assigned to tokens in the mask block. In the default setting, referred to as Aligned RoPE, each mask token copies the position id of its corresponding token in the reference context, so the two tokens share the same rotary position embedding. In the Without Aligned RoPE setting, mask tokens are instead assigned position ids according to their physical locations in the concatenated sequence, continuing after the reference context rather than reusing the data-token positions.

Table~\ref{tab:share-mask-position-ablation} shows that sharing RoPE positions between each mask token and its paired data token is crucial for valid target verification. Without aligned RoPE, GSM8K accuracy drops from $84.0\%$ to $0.0\%$, while the token-level acceptance rate also decreases substantially from $0.902$ to $0.718$. The large KL divergence of $7.12$ further indicates that physically continued position ids break the intended temporal verification geometry.
\input{src/table/rope_ablation}

==> neurips26_dllm_causal_mask/src/section/5_discussion.tex <==
\section{Conclusion}
%we identify a key incompatibility between diffusion large language models (dLLMs) and standard token-level speculative decoding. %Although dLLMs provide attractive parallelism through masked denoising and blockwise decoding, their bidirectional masked language modeling formulation does not preserve temporally valid token-level contexts across generation steps. As a result, vanilla dLLMs cannot directly verify multiple drafted tokens in a single forward pass, unlike autoregressive models, where speculative decoding accelerates inference by drafting and verifying multiple tokens in parallel. To address this challenge, 
%In this paper, we propose the \textbf{Token-Level Temporal Causal Mask}, a plug-and-play masking strategy that restores token-level temporal structure for dLLMs. By introducing reference tokens from draft-model predictions and designing an attention mask to control their interaction with current-step tokens, our method enables dLLMs to compute valid logits for drafted tokens under temporally consistent contexts. This brings the key verification ability of AR causal masking into dLLM decoding while preserving their parallel generation advantages. Since the method only modifies the attention mask and copies a small number of hidden states, it can be flexibly integrated with existing dLLM decoding pipelines and combined with other acceleration techniques such as KV caching and blockwise decoding.
%Extensive experiments on SDAR-family dLLMs across GSM8K, MBPP, TriviaQA, and MMLU demonstrate the effectiveness of our method. Without additional training, it achieves up to \(7.46\times\) higher decoding throughput over the vanilla SDAR baseline with tensor parallelism, while maintaining generation quality and improving average task performance by \(+1.7\%\). 
In this paper, we propose \textbf{SimSD}, a simple but effective plug-and-play strategy that restores token-level temporal structure for supporting dLLMs to use speculative decoding for inference acceleration. By introducing reference tokens from draft-model predictions and controlling their interactions with current-step tokens through a tailored attention mask, our method enables dLLMs to compute valid logits for drafted tokens under temporally consistent contexts. This brings the core verification capability of AR speculative decoding, where multiple drafted tokens are verified in parallel by the target model, to dLLM inference while preserving their parallel generation advantages. Since our method only modifies the attention mask and copies a small number of hidden states, it can be seamlessly integrated into existing dLLM decoding pipelines and combined with acceleration techniques such as KV caching and blockwise decoding.
Extensive experiments on SDAR-family dLLMs across GSM8K, MBPP, TriviaQA, and MMLU demonstrate the effectiveness of our method. Without additional training, it achieves up to \(7.46\times\) higher decoding throughput than the vanilla SDAR baseline with tensor parallelism, while maintaining generation quality and improving average task performance by \(+1.7\%\).

==> neurips26_dllm_causal_mask/src/table/eos_bounded_quality_efficiency.tex <==
\begin{table}[h]
\centering
\small
\caption{Accuracy performance.
We report accuracy for GSM8K, TriviaQA, and MMLU, and pass@1 for MBPP.
Van. denotes vanilla decoding, SD denotes our method SimSD, BL denotes the block length and $\alpha$ denotes the token-level acceptance rate.}
\label{tab:pass1_sd_vanilla}
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.10}
\begin{tabular}{ccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{BL}}
& \multicolumn{3}{c}{\textbf{GSM8K}}
& \multicolumn{3}{c}{\textbf{MBPP}}
& \multicolumn{3}{c}{\textbf{TriviaQA}}
& \multicolumn{3}{c}{\textbf{MMLU}}
& \multicolumn{2}{c}{\textbf{Avg.}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
\cmidrule(lr){14-15}
& Van. & SD & $\alpha$
& Van. & SD & $\alpha$
& Van. & SD & $\alpha$
& Van. & SD & $\alpha$
& Van. & SD \\
\midrule
4
& \textbf{0.922} & 0.896 & 0.915
& \textbf{0.669} & 0.662 & 0.806
& 0.486 & \textbf{0.537} & 0.576
& 0.706 & \textbf{0.758} & 0.973
& 0.696 & \textbf{0.713} \\
8
& \textbf{0.906} & 0.894 & 0.867
& \textbf{0.642} & 0.634 & 0.731
& 0.471 & \textbf{0.503} & 0.519
& 0.704 & \textbf{0.760} & 0.949
& 0.681 & \textbf{0.698} \\
\bottomrule
\end{tabular}
\end{table}

==> neurips26_dllm_causal_mask/src/table/gamma.tex <==
\begin{wraptable}{r}{0.52\textwidth}
\centering
\small
\caption{Effect of $\gamma$ on GSM8K.
We evaluate different values of $\gamma$ using SDAR-1.7B-b8 as draft model and  SDAR-8B-b8 as target model with block length $B=8$ on GSM8K. TPS denotes generated tokens per second,
real-$\alpha$ denotes the realized token-level acceptance rate, and avg accept denotes
the average number of accepted tokens per verification step.}
\label{tab:gamma_effect_gsm8k}
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{0.52\textwidth}{!}{
\begin{tabular}{cccccc}
\toprule
$\gamma$ & Accuracy & TPS & real-$\alpha$ & Avg. accept & ms/block \\
\midrule
3
& 50.0\% & 55.14 & 0.834 & 4.54/8 & 90 \\
4
& 54.0\% & \textbf{74.40} & 0.887 & 4.93/8 & \textbf{71} \\
5
& 68.0\% & 51.17 & 0.909 & 4.98/8 & 104 \\
6
& 70.0\% & 62.94 & 0.933 & 5.31/8 & 89 \\
7
& 76.0\% & 51.92 & 0.948 & 5.61/8 & 113 \\
8
& \textbf{82.0\%} & 58.74 & \textbf{0.964} & \textbf{6.18/8} & 109 \\
\bottomrule
\end{tabular}
}
\end{wraptable}

==> neurips26_dllm_causal_mask/src/table/rope_ablation.tex <==
\begin{table}[h]
\centering
\small
\caption{RoPE Alignment Ablation.
We evaluate SDAR-1.7B-Chat as the draft model and SDAR-8B-Chat as the target model on GSM8K.
Acc. denotes accuracy, and KL denotes KL divergence averaged over the target output distributions.}
\label{tab:share-mask-position-ablation}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.10}

\begin{tabular}{lcccc}
\toprule
\textbf{Setting}
& \textbf{GSM8K Acc.} 
& \textbf{Token-level $\alpha$} 
& \textbf{Accepted / Block} 
& \textbf{KL(Default $\|$ $\cdot$)} \\
\midrule
With Aligned RoPE
& \textbf{84.0\%}
& \textbf{0.902}
& \textbf{3.61/4}
& \textbf{--} \\
Without Aligned RoPE
& 0.0\%
& 0.718
& 2.87/4
& 7.12 \\
\bottomrule
\end{tabular}

\end{table}

==> neurips26_dllm_causal_mask/src/table/throughput_main_results.tex <==
\begin{table}[h]
\centering
\small
\caption{Efficiency Performance.
We report decode tokens per second. 
S2D2 denotes self-speculative decoding for diffusion LLMs, and SD denotes our speculative decoding method.
Speedup is measured relative to Vanilla with tensor parallelism of size 2 under the same block size. BL denotes the block length. CG denotes CUDA Graph. Van. denotes vanilla decoding}
\label{tab:sd_pipe_fast_denoise_tp2_speedup}
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.10}

\begin{tabular}{clcccccc}
\toprule
\multirow{2}{*}{\textbf{BL}}
& \multirow{2}{*}{\textbf{Methods}}
& \multicolumn{5}{c}{\textbf{Decoded Tokens per Second}}
& \multirow{2}{*}{\textbf{Speedup}} \\
\cmidrule(lr){3-7}
& & \textbf{GSM8K} & \textbf{TriviaQA} & \textbf{MBPP} & \textbf{MMLU} & \textbf{Mean} & \\
\midrule

\multirow{4}{*}{4}
& Vanilla
& 10.0 & 11.4 & 11.4 & 5.59 & 9.6 & 1.00$\times$ \\
& Vanilla + CG
& 50.1 & 50.5 & 50.7 & 56.04 & 51.8 & 5.40$\times$ \\
& S2D2
& 54.8 & 28.3 & 47.7 & 32.3 & 40.8 & 4.25$\times$ \\
& \textbf{SimSD}
& \textbf{72.6} & \textbf{73.3} & \textbf{72.2} & \textbf{68.4} & \textbf{71.6} & \textbf{7.46$\times$} \\
\midrule

\multirow{4}{*}{8}
& Vanilla
& 15.3 & 20.4 & 18.7 & 6.21 & 15.2 & 1.00$\times$ \\
& Vanilla + CG
& 30.9 & 31.9 & 30.4 & 36.8 & 32.5 & 2.14$\times$ \\
& S2D2
& 57.6 & 30.0 & 50.2 & 28.0 & 41.5 & 2.74$\times$ \\
& \textbf{SimSD}
& \textbf{74.1} & \textbf{88.3} & \textbf{80.4} & \textbf{84.4} & \textbf{81.8} & \textbf{5.40$\times$} \\
\bottomrule
\end{tabular}
\end{table}

==> src/figure/cross_model_figure.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/cross_model.png}
  \caption{Token-level temporal causal attention. (a) A step map assigns each token a temporal decoding order. (b) The input is arranged as prompt, data, and mask tokens, with shared temporal labels and aligned positional encoding. (c) The attention mask enforces token-level temporal causality.}
  \label{fig:cross_model}
\end{figure}

==> src/figure/self_draft_figure.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{figures/self_draft.png}
  \caption{Self draft Distribution Analysis}
  \label{fig:self_draft}
\end{figure}
